Forest Density Estimation

We study graph estimation and density estimation in high dimensions, using a family of density estimators based on forest structured undirected graphical models. For density estimation, we do not assume the true distribution corresponds to a forest; rather, we form kernel density estimates of the bivariate and univariate marginals, and apply Kruskal's algorithm to estimate the optimal forest on held out data. We prove an oracle inequality on the excess risk of the resulting estimator relative to the risk of the best forest. For graph estimation, we consider the problem of estimating forests with restricted tree sizes. We prove that finding a maximum weight spanning forest with restricted tree size is NP-hard, and develop an approximation algorithm for this problem. Viewing the tree size as a complexity parameter, we then select a forest using data splitting, and prove bounds on excess risk and structure selection consistency of the procedure. Experiments with simulated data and microarray data indicate that the methods are a practical alternative to Gaussian graphical models.

==> fde-arxiv/gadget.tex <==
\begin{figure}[t]
\begin{center}
\begin{tabular}{c}
\psset{nodesep=0pt}
\psset{linewidth=1pt}
\def\xscale{27pt}
\def\yscale{\xscale}
\psset{xunit=\xscale}
\psset{yunit=\yscale}
\pspicture(-6,-5)(6,8)
\def\tri{\pspolygon[](-.433,-.25)(.433,-.25)(0,.5)}
\def\tril{
   \pspolygon[](-.433,-.25)(.433,-.25)(0,.5)
   \psline(0,-.25)(0,-1.15)
   \psline(-.216,.125)(-1.08,.625)
}
\def\trir{
   \pspolygon[](-.433,-.25)(.433,-.25)(0,.5)
   \psline(0,-.25)(0,-1.15)
   \psline(.216,.125)(1.08,.625)
}
\def\trit{
   \pspolygon[](-.433,-.25)(.433,-.25)(0,.5)
   \cnodeput(2.165,1.25){TCR}{$\;\;$}
   \cnodeput(-2.165,1.25){TCL}{$\;\;$}
   \pnode(.216,.125){TTR}
   \pnode(-.216,.125){TTL}
   \ncline{-}{TTR}{TCR}
   \ncline{-}{TTL}{TCL}
}
%\psgrid
\cnodeput(0,2.5){A}{$\;\;$}
\pnode(0,5){AA}
\rput(0,5.25){\trit}
\cnodeput(-2.17,-1.25){B}{$\;\;$}
\pnode(-4.33,-2.50){BB}
\rput(-4.54,-2.62){\tril}
\cnodeput(2.17,-1.25){C}{$\;\;$}
\pnode(4.33,-2.50){CC}
\rput(4.54,-2.62){\trir}
\rput(0,0){\psframe(-.4,-.4)(.4,.4)}
\pnode(0,.4){TC}
\pnode(-.36,-.2){BL}
\pnode(.36,-.2){BR}
\ncline{-}{TC}{A}
\ncline{-}{BL}{B}
\ncline{-}{BR}{C}
\ncline{-}{A}{AA}
\ncline{-}{B}{BB}
\ncline{-}{C}{CC}
\cnodeput[doubleline=true](1.13,.65){L1}{$\;$}
\cnodeput[doubleline=true](1.99,1.15){L2}{$\;$}
\cnodeput[doubleline=true](2.857,1.65){L3}{$\;$}
\pnode(0.3897114,0.2250000){L0}
\ncline{-}{L0}{L1}
\ncline{-}{L1}{L2}
\ncline{-}{L2}{L3}
\psccurve[linestyle=dashed,linecolor=blue,showpoints=false](-3,-2)(3,-2)(3,3)(-3,3)
\pscurve[linestyle=dashed,linecolor=blue,showpoints=false](2.0,5.2)(1,5.8)(.8,7)
\pscurve[linestyle=dashed,linecolor=blue,showpoints=false](-2.0,5.2)(-1,5.8)(-.8,7)
\rput(0,7.6){other gadgets}
\rput(4,3){gadget}
\rput(-1.5,2){$\stackrel{\mbox{\small nexus}}{\mbox{\small node}}$}
\rput(-2.5,.3){$\stackrel{\mbox{\small junction}}{\mbox{\small node}}$}
\rput(2.5,-3.5){$\stackrel{\mbox{\small element}}{\mbox{\small node}}$}
\rput(2.65,-.08){$\mbox{\small lures}$}
\psline[linewidth=.7pt]{->}(3.3,-3.4)(4,-3)
\psline[linewidth=.7pt]{->}(2.6,.2)(1.5,.5)
\psline[linewidth=.7pt]{->}(2.6,.2)(2.2,.8)
\psline[linewidth=.7pt]{->}(2.6,.2)(2.8,1.2)
\psline[linewidth=.7pt]{->}(-1.1,1.6)(-.4,.6)
\psline[linewidth=.7pt]{->}(-2.5,-.1)(-2.3,-.85)
\rput(-1.2,6.2){\fs 2}
\rput(1.2,6.2){\fs 2}
\rput(.2,3.8){\fs 2}
\rput(3.1,-1.5){\fs 2}
\rput(-3.1,-1.5){\fs 2}
\rput(0.3,1.4){\fs $N$}
\rput(-1.0,-0.9){\fs $N$}
\rput(1.0,-0.9){\fs $N$}
\rput(0.55,0.6){\fs 5}
\rput(1.45,1.1){\fs 10}
\rput(2.35,1.6){\fs 10}
\endpspicture
\end{tabular}
\end{center}
\vskip-30pt
\caption{Gadget constructed in the reduction from X3C}
\label{fig:gadget}
\end{figure}

